Learning Graphs from Smooth and Graph-Stationary Signals with Hidden Variables

Network-topology inference from (vertex) signal observations is a prominent problem across data-science and engineering disciplines. Most existing schemes assume that observations from all nodes are available, but in many practical environments, only a subset of nodes is accessible. A natural (and sometimes effective) approach is to disregard the role of unobserved nodes, but this ignores latent network effects, deteriorating the quality of the estimated graph. Differently, this paper investigates the problem of inferring the topology of a network from nodal observations while taking into account the presence of hidden (latent) variables. Our schemes assume the number of observed nodes is considerably larger than the number of hidden variables and build on recent graph signal processing models to relate the signals and the underlying graph. Specifically, we go beyond classical correlation and partial correlation approaches and assume that the signals are smooth and/or stationary in the sought graph. The assumptions are codified into different constrained optimization problems, with the presence of hidden variables being explicitly taken into account. Since the resulting problems are ill-conditioned and non-convex, the block matrix structure of the proposed formulations is leveraged and suitable convex-regularized relaxations are presented. Numerical experiments over synthetic and real-world datasets showcase the performance of the developed methods and compare them with existing alternatives.

==> backup.tex <==
Expressing in block matrix form $\bbX$, the GSO $\bbS$ and the covariance matrix $\bbC = \mathbb{E}[\bbX\bbX^{T}] \in \mathbb{R}^{N \times N}$ of the random graph process we have the following expressions respectively
\begin{equation}\label{E:block_XSC}
    \bbX \!=\!
    \begin{bmatrix}
    \bbX_O \\
    \bbX_{H}
    \end{bmatrix}, \;
    \bbS \!=\!
    \begin{bmatrix}
    \bbS_O & \bbS_{OH}  \\
    \bbS_{OH}^T & \bbS_H
    \end{bmatrix}, \;
    \bbC \!=\!
    \begin{bmatrix}
    \bbC_O & \bbC_{OH}  \\
    \bbC_{OH}^T & \bbC_H
    \end{bmatrix}\!.
\end{equation}
%

The division by matrix blocks shown above, allows us to understand $\bbX$ by its observed part $\bbX_{O} \in \mathbb{R}^{O \times M}$ but knowing that there is a hidden block $\bbX_{H} \in \mathbb{R}^{H \times M}$.\sre{por qué es importante para formular el problema?}
%influencia que tienen
%un problema mas complicado
Note that this fact is important because from block matrix $\bbX$ can be obtained the covariance block matrix as $\bbC_{O} = \mathbb{E}[\bbX_{O}\bbX_{O}^{T}]$, $\bbC_{OH} = \mathbb{E}[\bbX_{O}\bbX_{H}^{T}]$ and similarly for the other blocks.
The same block structure from the covariance matrix is applied for the GSO $\bbS$ which is showing in (\ref{E:block_XSC}).
\sre{Por qué es necesaria la C? Si la defines aquí explica por qué nos importa, si no, defínela cuando la usemos.}
Then, the submatrices $\bbS_{O}$ and $\bbC_{O}$, both of dimension $O \times O$, are associated with the observed variables while the other blocks are related to hidden variables.
When models to solve the inference problem are proposed it is necessary to realize that the size of $\bbX$ depends on the number of available realizations for each node, $M \gg N$ which affects directly to the time execution of the implemented algorithms.
To facilitate the problem statement and make our algorithms faster, we will use the covariance of the observed signals $\bbC_{O}$ instead of $\bbX_{O}$.
Here we introduce the hidden variables in $\bbX$, $\bbS$ and $\bbC$ because in the next sections will be used to adapt the topology inference problems when the presence of hidden variables is considered for particular scenarios.\sre{Aunque esta frase no está mal, algo hay que decir de las ocultas. Por qué es conveniente introducirlas? Que implica?}
%This formulation will be used in the following sections to solve the topology inference problem in the presence of hidden variables.

In this paper we investigate how to use signals $\bbX_{O}$ to infer $\bbS_{O}$ while taking into account the effect of the hidden variables, which makes the inference problem to gain a lot of degrees of freedom and makes it ill-conditioned. 
To deal with this issues it is necessary to solve the inference problem under strong assumptions that relate the properties of the signals to those of the underlying graph.
%\sre{Las strong assumptions ligan con el comentario anterior, hacen falta porque el problema gana demasiados grados de libertad.}
In particular, we will study two different scenarios: (i) smooth signals over the graph; and (ii) stationary signals in $\bbS$.
